LLM-Rec: Personalized Recommendation via Prompting Large Language Models

Text-based recommendation holds a wide range of practical applications due to its versatility, as textual descriptions can represent nearly any type of item. However, directly employing the original item descriptions may not yield optimal recommendation performance due to the lack of comprehensive information to align with user preferences. Recent advances in large language models (LLMs) have showcased their remarkable ability to harness commonsense knowledge and reasoning. In this study, we introduce a novel approach, coined LLM-Rec, which incorporates four distinct prompting strategies of text enrichment for improving personalized text-based recommendations. Our empirical experiments reveal that using LLM-augmented text significantly enhances recommendation quality. Even basic MLP (Multi-Layer Perceptron) models achieve comparable or even better results than complex content-based methods. Notably, the success of LLM-Rec lies in its prompting strategies, which effectively tap into the language model's comprehension of both general and specific item characteristics. This highlights the importance of employing diverse prompts and input augmentation techniques to boost the recommendation effectiveness of LLMs.

==> tab_fig/comp_different_prompt.tex <==
\begin{table*}[h]
\adjustbox{max width=\textwidth}{
\begin{tabular}{llllllll}
\toprule
                             &                   &              & \textbf{Movielens-1M} &         &              & \textbf{Recipe}    &         \\
                             &                   & Precision@10 & Recall@10    & NDCG@10 & Precision@10 & Recall@10 & NDCG@10 \\\midrule
\multicolumn{2}{l}{Content Description} & 0.2922 \scriptsize{$\textcolor{gray}{\pm 0.0019}$}& 0.2455 \scriptsize{$\textcolor{gray}{\pm 0.0031}$}& 0.3640 \scriptsize{$\textcolor{gray}{\pm 0.0039}$}& 0.0325 \scriptsize{$\textcolor{gray}{\pm 0.0021}$}& 0.0684 \scriptsize{$\textcolor{gray}{\pm 0.0066}$}& 0.0580 \scriptsize{$\textcolor{gray}{\pm 0.0054}$} \\\midrule
\multirow{8}{*}{{\sc Llama-2}}     & ${\tt p_{para}}$           &              &              &         &              &           &         \\
                             & ${\tt p_{tag}}$            &              &              &         &              &           &         \\
                             & ${\tt p_{infer}}$          &              &              &         &              &           &         \\
                             & ${\tt p_{para}^{rec}}$      &              &              &         &              &           &         \\
                             & ${\tt p_{tag}^{rec}}$       &              &              &         &              &           &         \\
                             & ${\tt p_{infer}^{rec}}$     &              &              &         &              &           &         \\
                             & ${\tt p^{eng}}$           &              &              &         &              &           &         \\
                             & ${\tt p^{rec+eng}}$        &              &              &         &              &           &         \\\midrule
\multirow{8}{*}{{\sc GPT-3}}       & ${\tt p_{para}}$           &              &              &         &              &           &         \\
                             & ${\tt p_{tag}}$            &              &              &         &              &           &         \\
                             & ${\tt p_{infer}}$          &              &              &         &              &           &         \\
                             & ${\tt p_{para}^{rec}}$      &              &              &         &              &           &         \\
                             & ${\tt p_{tag}^{rec}}$       &              &              &         &              &           &         \\
                             & ${\tt p_{infer}^{rec}}$     &              &              &         &              &           &         \\
                             & ${\tt p^{eng}}$            &              &              &         &              &           &         \\
                             & ${\tt p^{rec+eng}}$         &              &              &         &              &           &    \\\bottomrule    
\end{tabular}
}
\end{table*}

==> tab_fig/figure_llm-rec.tex <==
\begin{figure*}[htbp]
    \begin{center}
    \includegraphics[width=\linewidth]{figure/llm_rec_framework.pdf}
    \end{center}
    \caption{\model plays a crucial role in enabling large language models to provide relevant context and help better align with user preferences. Prompts and augmented texts are highlighted.}
    \label{fig:llm-rec}
\end{figure*}

==> tab_fig/intro_res_figure.tex <==

\begin{figure}[t]
% \vspace{-.5cm}
\vspace{-2mm}
    \begin{center}
    \includegraphics[width=\linewidth]{figure/intro.pdf}
    \vspace{-10mm}
    \end{center}
      \caption{\model enriches original item descriptions via various prompting strategies. Integrating the augmented text as the new input achieves comparable or even superior recommendation performance compared to both the baseline model (\ie MLP) and more advanced content-based models like DCN-V2~\citep{wang2021dcn} that rely solely on the original item description.}\label{fig:intro_fig}
      \vspace{-5mm}
\end{figure}
